Angular distribution of $\gamma$ rays from the p-wave resonance of $^{118}$Sn

The neutron energy-dependent angular distribution of $\gamma$ rays from $^{117}{\rm Sn}(n,\gamma)$ reaction was measured with germanium detectors and a pulsed neutron beam. The angular distribution was clearly observed in $\gamma$-ray emissions with an energy of 9327 keV which corresponds to the transition from a neutron resonance of $^{117}{\rm Sn}+n$ to the ground state of $^{118}{\rm Sn}$. The angular distribution causes an angular-dependent asymmetric resonance shape. An asymmetry $A_{\rm LH}$ was defined as $(N_{\rm L}-N_{\rm H})/(N_{\rm L}+N_{\rm H})$, where $N_{\rm L}$ and $N_{\rm H}$ are integrated values for lower- and higher-energy regions of a neutron resonance, respectively. We found that the $A_{\rm LH}$ has the angular dependence of $(A \cos \theta_\gamma +B)$, where $\theta_\gamma$ is the $\gamma$-ray emission angle with respect to the incident neutron momentum, with $A=0.394 \pm 0.073$ and $B = 0.118 \pm 0.029$ in the 1.33 eV p-wave resonance.

==> sections/section04_old.tex <==
\section{Discussion} \label{sec:discussion}

To evaluate the $E^{\rm m}_n$ dependence of the angular distribution of $\gamma$ rays, the cross section of the (n,$\gamma$) reaction for unpolarized neutron is expanded by using Legendre polynomial up to the second order for the $\gamma$-ray emission angle $\theta_\gamma$
\begin{align}
    \frac{d\sigma}{d\Omega} = c_0 + c_1 \cdot \cos\theta_\gamma + c_2 \cdot \frac{1}{2} \left(\cos^2\theta_\gamma - \frac{1}{3} \right),
    \label{eq:LegendrePolynomial}
\end{align}
where $c_0$, $c_1$, and $c_2$ depend on both $E_n$ and $\theta_\gamma$.
Using the integrated values in the lower energy region $N_{\rm L}(\theta_\gamma)$ and in the higher energy region $N_{\rm H}(\theta_\gamma)$ than the resonance energy $E_{\rm p}$ of the p-wave resonance, we consider the following equation;
\begin{align}
    N_{\rm L}(\theta_\gamma) - N_{\rm H}(\theta_\gamma) =& (c_{0,{\rm L}} - c_{0,{\rm H}}) + (c_{1,{\rm L}} - c_{1,{\rm H}}) \cdot \cos\theta_\gamma \nonumber \\ &+ (c_{2,{\rm L}} - c_{2,{\rm H}}) \cdot \frac{1}{2} \left(\cos^2\theta_\gamma - \frac{1}{3} \right),
    \label{eq:NLmNH}
\end{align}
\begin{align}
    N_{\rm L}(\theta_\gamma) + N_{\rm H}(\theta_\gamma) =& (c_{0,{\rm L}} + c_{0,{\rm H}}) + (c_{1,{\rm L}} + c_{1,{\rm H}}) \cdot \cos\theta_\gamma \nonumber \\ &+ (c_{2,{\rm L}} + c_{2,{\rm H}}) \cdot \frac{1}{2} \left(\cos^2\theta_\gamma - \frac{1}{3} \right).
    \label{eq:NLpNH}
\end{align}
Here, the subscripts L and H represent "low energy region" and "high energy region", respectively.
Figures~\ref{fig:NLmNH} and \ref{fig:NLpNH} show $N_{\rm L}(\theta_\gamma)-N_{\rm H}(\theta_\gamma)$ and $N_{\rm L}(\theta)+N_{\rm H}(\theta_\gamma)$ plots as functions of $\cos\theta_\gamma$, respectively.
The regions for integration were defined using the p-wave resonance energy $E_{\rm p}$ and the total resonance width $\Gamma_{\rm p}$ as follows;
$E_{\rm p}-2\Gamma_{\rm p} < E_n < E_{\rm p}$ for $N_{\rm L}(\theta)$ and $E_{\rm p} < E_n < E_{\rm p}+2\Gamma_{\rm p}$ for $N_{\rm H}(\theta)$.
The total resonance width is defined as $\Gamma_{\rm p} = \Gamma^\gamma_{\rm p} + \Gamma^n_{\rm p}$.
Here, the resonance parameters, $E_{\rm p}$, $\Gamma^\gamma_{\rm p}$, and $\Gamma^n_{\rm p}$, were the values described in Table~\ref{tab:ResonanceParameter}.
%Figure: NL-NH
\begin{figure}[tbp]
    \centering
    \includegraphics[width=.45\textwidth]{./figure/NLminusNH.eps}
    \caption{Angular dependence of $N_{\rm L}(\theta_\gamma) - N_{\rm H}(\theta_\gamma)$ as a function of $\cos\theta_\gamma$. It is clear that the angular dependence of this plot is linear.}
    \label{fig:NLmNH}
\end{figure}
%Figure: NL-NH
%Figure: NL+NH
\begin{figure}[tbp]
    \centering
    \includegraphics[width=.45\textwidth]{./figure/NLplusNH.eps}
    \caption{Angular dependence of $N_{\rm L}(\theta_\gamma) + N_{\rm H}(\theta_\gamma)$ as a function of $\cos\theta_\gamma$.}
    \label{fig:NLpNH}
\end{figure}
%Figure: NL+NH
Figure~\ref{fig:NLmNHfit} shows the best fit of $N_{\rm L}(\theta_\gamma) - N_{\rm H}(\theta_\gamma)$ with the polynomial function up to the first order with $\theta_\gamma$ as a variable for Fig.~\ref{fig:NLmNH}.
The fitting parameters were obtained as
\begin{align}
    c_0 = 0.762 \pm 0.193 ~{\rm and}~ c_1 = 2.780 \pm 0.470 . \nonumber
\end{align}
This fitting result indicates that the angular dependence of $N_{\rm L}(\theta_\gamma) - N_{\rm H}(\theta_\gamma)$ is linear.

Therefore, the second order in Eq.~(\ref{eq:NLmNH}) is negligible.
%Figure: NL-NH fitting
\begin{figure}[tbp]
    \centering
    \includegraphics[width=.45\textwidth]{./figure/NLminusNH_fit.eps}
    \caption{Fitting result for determining the angular-dependent parameters of Legendre polynomial for $N_{\rm L}(\theta_\gamma) - N_{\rm H}(\theta_\gamma)$.}
    \label{fig:NLmNHfit}
\end{figure}
%Figure: NL-NH fitting
%Figure: NL+NH fitting
\begin{figure}[tbp]
    \centering
    \includegraphics[width=.45\textwidth]{./figure/NLplusNH_fit.eps}
    \caption{Fitting result for determining the angular-dependent parameters of Legendre polynomial for $N_{\rm L}(\theta_\gamma) + N_{\rm H}(\theta_\gamma)$. The coefficients of angular-dependent terms are zero within statistical errors.}
    \label{fig:NLpNHfit}
\end{figure}
%Figure: NL+NH fitting
Figure~\ref{fig:NLpNHfit} shows the fitting result with a polynomial function up to the second order with $\theta_\gamma$ as a variable for Fig.~\ref{fig:NLpNH}.
The fitting parameters were obtained as
\begin{align*}
    c_0 &= 6.564 \pm 0.232 ,\\
    c_1 &= -0.427 \pm 0.511 ,\\
    c_2 &= 0.740 \pm 0.872 .
\end{align*}
The coefficients of angular-dependent terms are zero within statistical errors, which implies that Eq.~(\ref{eq:NLpNH}) has no angular dependence and can be regarded as a constant.
Therefore, the $E^{\rm m}_n$ dependence of the angular distribution can be evaluated by the asymmetry $A_{\rm LH}(\theta_\gamma)$ which is defined as 
\begin{align}
    A_{\rm LH}(\theta_\gamma) = \frac{N_{\rm L}(\theta_\gamma) - N_{\rm H}(\theta_\gamma)}{N_{\rm L}(\theta_\gamma) + N_{\rm H}(\theta_\gamma)},
\end{align}
and this asymmetry can be parameterized as 
\begin{align}
    A_{\rm LH}(\theta_\gamma) = A\cos\theta_\gamma + B.
    \label{eq:AsymmetryParameter}
\end{align}


The asymmetry $A_{\rm LH}(\theta_\gamma)$ can be fitted using Eq.~(\ref{eq:AsymmetryParameter}), and the fitting result is shown in Fig.~\ref{fig:Asym_fixedfit}.
The parameters of the $A_{\rm LH}(\theta_\gamma)$ were obtained as
\begin{align}
A = 0.394 \pm 0.073 ~{\rm and}~ B = 0.118 \pm 0.029.
\end{align}
This indicates the $E^{\rm m}_n$ dependence of the angular distribution is linear correlation.
%Future measurements of other angular-dependent terms with polarized and unpolarized neutron beam may verify the $sp$-mixing model of compound states.
\begin{figure}[htbp]
    \centering
%    \includegraphics[width=.45\textwidth]{./figure/Asym_FixedFit.eps}
    \includegraphics[width=.45\textwidth]{./figure/AsymmetryFit.eps}
    \caption{Fitting result for $A_{\rm LH}(\theta_\gamma)$ using Eq.~(\ref{eq:AsymmetryParameter}). The angular-dependent parameter $A$ were obtained to be a significant value.}
    \label{fig:Asym_fixedfit}
\end{figure}
